Applications of Random Graphs to 2D Quantum Gravity

The central topic of this thesis is two dimensional Quantum Gravity and its properties. The term Quantum Gravity itself is ambiguous as there are many proposals for its correct formulation and none of them have been verified experimentally. In this thesis we consider a number of closely related approaches to two dimensional quantum gravity that share the property that they may be formulated in terms of random graphs. In one such approach known as Causal Dynamical Triangulations, numerical computations suggest an interesting phenomenon in which the effective spacetime dimension is reduced in the UV. In this thesis we first address whether such a dynamical reduction in the number of dimensions may be understood in a simplified model. We introduce a continuum limit where this simplified model exhibits a reduction in the effective dimension of spacetime in the UV, in addition to having rich cross-over behaviour. In the second part of this thesis we consider an approach closely related to causal dynamical triangulation; namely dynamical triangulation. Although this theory is less well-behaved than causal dynamical triangulation, it is known how to couple it to matter, therefore allowing for potentially multiple boundary states to appear in the theory. We address the conjecture of Seiberg and Shih which states that all these boundary states are degenerate and may be constructed from a single principal boundary state. By use of the random graph formulation of the theory we compute the higher genus amplitudes with a single boundary and find that they violate the Seiberg-Shih conjecture. Finally we discuss whether this result prevents the replacement of boundary states by local operators as proposed by Seiberg.

==> abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                              ABSTRACT                               %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\baselineskip = 12pt plus 1pt minus 1pt

\centerline{\large Applications of Random Graphs to 2D Quantum Gravity}
\vspace{ 1.0cm }
\centerline{\large Max Atkin}
\vspace{0.2cm}
\centerline{\large Christ Church, Oxford}

\vspace{0.6cm}
\centerline{submitted for the degree of Doctor of Philosophy}
\centerline{at the University of Oxford}
\vspace{0.5cm}
\centerline{Trinity Term, 2011}
\vspace{1.0cm }
{ \large \bf \centerline {ABSTRACT} }
\addcontentsline{toc}{chapter}{Abstract} 
\vspace{ 1.0cm }
The central topic of this thesis is two dimensional Quantum Gravity and its properties. The term Quantum Gravity itself is ambiguous as there are many proposals for its correct formulation and none of them have been verified experimentally. In this thesis we consider a number of closely related approaches to two dimensional quantum gravity that share the property that they may be formulated in terms of random graphs.
In one such approach known as Causal Dynamical Triangulations, numerical computations suggest an interesting phenomenon in which the effective spacetime dimension is reduced in the UV. In this thesis we first address whether such a dynamical reduction in the number of dimensions may be understood in a simplified model. We introduce a continuum limit where this simplified model exhibits a reduction in the effective dimension of the spacetime in the UV, in addition to having rich cross-over behaviour.

In the second part of this thesis we consider an approach closely related to causal dynamical triangulation; namely dynamical triangulation. Although this theory is less well-behaved than causal dynamical triangulation, it is known how to couple it to matter, therefore allowing for potentially mulitple boundary states to appear in the theory. We address the conjecture of Seiberg and Shih which stated that all these boundary states are degenerate and may be constructed from a single principal boundary state. By use of the random graph formulation of the theory we compute the higher genus amplitudes with a single boundary and find that they violate the Seiberg-Shih conjecture. Finally we discuss whether this result prevents the replacement of boundary states by local operators as proposed Seiberg.  



==> dedic.tex <==
\vspace{4cm}
\begin{center}
{\bf For Lauren and my Family}
\end{center}
\vspace{20cm}
\begin{flushright}
\end{flushright}



==> jfchrs2e.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
%                                PJCHRS.TEX                               %
%                                                                         %
%                            (For use in CERNTEX)                         %
%                                                                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MATHS STUFF %
\newcommand{\approxgt}{\mbox{\raisebox{-.5ex}\ensuremath{\stackrel{>}{\sim}}}}
\newcommand{\approxlt}{\mbox{\raisebox{-.5ex}\ensuremath{\stackrel{<}{\sim}}}}
\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\mod}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}}
\newcommand{\s}{\ensuremath{\sim}}
\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\lra}{\ensuremath{\leftrightarrow}}
\newcommand{\longra}{\ensuremath{\longrightarrow}}
\newcommand{\mstrut}{\rule{0cm}{5ex}}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\tc}[1]{\ensuremath{\tiny #1}}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}}

% FRACTIONS%
\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\third}{\ensuremath{\frac{1}{3}}}
\newcommand{\quarter}{\ensuremath{\frac{1}{4}}}
\newcommand{\fifth}{\ensuremath{\frac{1}{5}}}
\newcommand{\sixth}{\ensuremath{\frac{1}{6}}}
\newcommand{\seventh}{\ensuremath{\frac{1}{7}}}
\newcommand{\eighth}{\ensuremath{\frac{1}{8}}}
\newcommand{\ninth}{\ensuremath{\frac{1}{9}}}
\newcommand{\tenth}{\ensuremath{\frac{1}{10}}}
\newcommand{\twelfth}{\ensuremath{\frac{1}{12}}}
\newcommand{\sixteenth}{\ensuremath{\frac{1}{16}}}


% BOLDMATHS SYMBOLS %

\newcommand{\bmW}{\ensuremath{\mathbf{W}}}
\newcommand{\bmF}{\ensuremath{\mathbf{F}}}
\newcommand{\bmX}{\ensuremath{\mathbf{X}}}
\newcommand{\bmI}{\ensuremath{\mathbf{I}}}
\newcommand{\bmalpha}{\ensuremath{\boldmath{\alpha}}}
\newcommand{\bmtheta}{\ensuremath{\mathbf{\theta}}}
\newcommand{\bmsigma}{\ensuremath{\mathbf{\sigma}}}
\newcommand{\bmlambda}{\ensuremath{\mathbf{\lambda}}}
\newcommand{\bmtau}{\ensuremath{\mathbf{\tau}}}
\newcommand{\bmdag}{\ensuremath{\mathbf{\dagger}}}

% COORDINATES %
\newcommand{\Delx}{\ensuremath{\Delta x}}
\newcommand{\Dely}{\ensuremath{\Delta y}}
\newcommand{\rphi}{\ensuremath{r-\phi}}
\newcommand{\sz}{\ensuremath{s-z}}
\newcommand{\xy}{\ensuremath{x-y}}
\newcommand{\zo}{\ensuremath{z_0}}
\newcommand{\modzo}{\ensuremath{\left| z_0 \right|}}
\newcommand{\meanzo}{\ensuremath{\left\langle z_0 \right\rangle}}
\newcommand{\bphi}{\ensuremath{\bar\phi}}
\newcommand{\bthe}{\ensuremath{\bar\theta}} 

% CHI SQUAREDS %
\newcommand{\chisq}{\ensuremath{{\chi}^2}}

% GROUPS %
\newcommand{\grpsuth}{\ensuremath{\mathrm{SU}(3)}}
\newcommand{\grpsutw}{\ensuremath{\mathrm{SU}(2)}}
\newcommand{\grpuone}{\ensuremath{\mathrm{U}(1)}}

% PARTICLES %
\newcommand{\qqbar}{\ensuremath{q{\bar q}}}
\newcommand{\ffbar}{\ensuremath{f{\bar f}}}
\newcommand{\bbbar}{\ensuremath{b{\bar b}}}
\newcommand{\ccbar}{\ensuremath{c{\bar c}}}
\newcommand{\ee}{\ensuremath{e^{+}e^{-}}}
\newcommand{\mumu}{\ensuremath{\mu^{+}\mu^{-}}}
\newcommand{\tautau}{\ensuremath{\tau^{+}\tau^{-}}}
\newcommand{\eemm}{\ensuremath{\ee \ra \mumu}}
\newcommand{\eemmg}{\ensuremath{\ee \ra \mumu (\gamma)}}
\newcommand{\eemmng}{\ensuremath{\ee \ra \mumu ( \mathrm{n} \gamma)}}
\newcommand{\eett}{\ensuremath{\ee \ra \tautau}}
\newcommand{\eeee}{\ensuremath{\ee \ra \ee}}
\newcommand{\nmu}{\ensuremath{\nu_{\mu}}}
\newcommand{\nbmu}{\ensuremath{{\overline{\nu}}_{\mu}}}
\newcommand{\nel}{\ensuremath{\nu_{e}}}
\newcommand{\nbel}{\ensuremath{{\overline{\nu}}_{e}}}
\newcommand{\ntau}{\ensuremath{\nu_{\tau}}}
\newcommand{\nbtau}{\ensuremath{{\overline{\nu}}_{\tau}}}
\newcommand{\ppos}{\ensuremath{\pi^{+}}}
\newcommand{\pneg}{\ensuremath{\pi^{-}}}
\newcommand{\pzer}{\ensuremath{\pi^{0}}}
\newcommand{\ppm}{\ensuremath{\pi^{\pm }}}
\newcommand{\Zo}{\ensuremath{\mathrm{Z}^0}}
\newcommand{\Zostar}{\ensuremath{\mathrm{Z}^{0\ast}}}
\newcommand{\Wpm}{\ensuremath{\mathrm{W}^\pm}}
\newcommand{\Ho}{\ensuremath{\mathrm{H}^0}}
% STANDARD MODEL PARAMS %
\newcommand{\MZ}{\ensuremath{\mathrm{M_Z}}}
\newcommand{\GZ}{\ensuremath{\Gamma_{\mathrm{Z}}}}
\newcommand{\TZ}{\ensuremath{\tau_{\mathrm{Z}}}}
\newcommand{\MW}{\ensuremath{\mathrm{M_W}}}
\newcommand{\MH}{\ensuremath{\mathrm{M_H}}}
\newcommand{\mt}{\ensuremath{\mathrm{m_t}}}
\newcommand{\ssqtw}{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}
\newcommand{\csqtw}{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}
\newcommand{\stw}{\ensuremath{\sin\theta_{\mathrm{W}}}}
\newcommand{\ctw}{\ensuremath{\cos\theta_{\mathrm{W}}}}
\newcommand{\ssqtwef}{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}
\newcommand{\csqtwef}{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}
\newcommand{\stwef}{\\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}
\newcommand{\ctwef}{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}
\newcommand{\gv}{\ensuremath{g_{\mbox{\tiny V}}}}
\newcommand{\ga}{\ensuremath{g_{\mbox{\tiny A}}}}
\newcommand{\gvel}{\ensuremath{g_{\mathrm{V}}^{e}}}
\newcommand{\gael}{\ensuremath{g_{\mathrm{A}}^{e}}}
\newcommand{\gvmu}{\ensuremath{g_{\mathrm{V}}^{\mu}}}
\newcommand{\gamu}{\ensuremath{g_{\mathrm{A}}^{\mu}}}
\newcommand{\gvf}{\ensuremath{g_{\mathrm{V}}^{f}}}
\newcommand{\gaf}{\ensuremath{g_{\mathrm{A}}^{f}}}
\newcommand{\ghvf}{\ensuremath{\hat{g}_{\mathrm{V}}^{f}}}
\newcommand{\ghaf}{\ensuremath{\hat{g}_{\mathrm{A}}^{f}}}
\newcommand{\thw}{\ensuremath{\theta_{\mbox{\mathrm{W}}}}}
\newcommand{\GF}{\ensuremath{G_{\mbox{\tiny F}}}}
\newcommand{\Vub}{\ensuremath{\mathrm{V}_{ub}}}
\newcommand{\Vcb}{\ensuremath{\mathrm{V}_{cb}=}}

% ORDERS %
\newcommand{\ordalph}{\ensuremath{\mathcal{O}(\alpha)}}
\newcommand{\ordalsq}{\ensuremath{\cal{O}(\alpha^{2})}}
% OBSERVABLES %
%\newcommand{\Afb}{\ensuremath{A_\mathrm{fb}}}
\newcommand{\sigmm}{\ensuremath{\sigma^{\mu\mu}}}
\newcommand{\sigtot}{\ensuremath{\sigma_{\mbox{\tiny TOT}}}}
\newcommand{\sigf}{\ensuremath{\sigma_{\mbox{\tiny F}}}}
\newcommand{\sigb}{\ensuremath{\sigma_{\mbox{\tiny B}}}}
\newcommand{\dsigf}{\ensuremath{\delta\sigma_{\mbox{\tiny F}}}}
\newcommand{\dsigb}{\ensuremath{\delta\sigma_{\mbox{\tiny B}}}}
\newcommand{\AFB}{\ensuremath{A_{\mbox{\tiny FB}}}}
\newcommand{\AFBmm}{\ensuremath{A_{\mbox{\tiny FB}}^{\mu\mu}}}
\newcommand{\APOL}{\ensuremath{A_{\mbox{\tiny POL}}}}
\newcommand{\pwff}{\ensuremath{\Gamma_{ff}}}
\newcommand{\pwee}{\ensuremath{\Gamma_{ee}}}
\newcommand{\pwmm}{\ensuremath{\Gamma_{\mu\mu}}}
\newcommand{\Af}{\ensuremath{\cal{A}_{f}}}
\newcommand{\Ael}{\ensuremath{\cal{A}_{e}}}
\newcommand{\Amu}{\ensuremath{\cal{A}_{\mu}}}
\newcommand{\dafbint}{\ensuremath{\delta A_{\mbox{\tiny FB}}^{\mbox{\tiny int}}}}
\newcommand{\Nch}{\ensuremath{\mathrm{N}_{\mathrm{ch}}}}
%Impact parameters
\newcommand{\IPRPHI}{\ensuremath{\mathrm{IP}_{R\phi}}}
\newcommand{\IPZ}{\ensuremath{\mathrm{IP}_{z}}}

% KINEMATICS %
\newcommand{\Ephot}{\ensuremath{E_{\gamma}}}
\newcommand{\Ebeam}{\ensuremath{E_{\mbox{\tiny BEAM}}}}
\newcommand{\sprime}{\ensuremath{s^{\prime}}}
\newcommand{\sqs}{\ensuremath{\sqrt{s}}}
\newcommand{\sqsp}{\ensuremath{\sqrt{\sprime}}}
%\newcommand{\pT}{\ensuremath{p_{\tiny T}}}
\newcommand{\pT}{\ensuremath{\mathrm{p_T}}}
\newcommand{\mmu}{\ensuremath{m_{\mu}}}
\newcommand{\mb}{\ensuremath{m_{b}}}
\newcommand{\thacop}{\ensuremath{\theta_{acop}}}
\newcommand{\thacol}{\ensuremath{\theta_{acol}}}

% UNITS %
\newcommand{\dgr}{\ensuremath{^\circ}}
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}}
\newcommand{\MeV}{\ensuremath{\mathrm{MeV}}}
\newcommand{\umm}{\ensuremath{\mu{\mathrm m}}}
\newcommand{\mrad}{\ensuremath{\mathrm{mrad}}}
% SPECIAL TEXT %
\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\etal}{{\sl et al\/}\ }
\newcommand{\KORALZ}{\mbox{\tt KORALZ}}
\newcommand{\ZFITTER}{\mbox{\tt ZFITTER}}
\newcommand{\DELANA}{\mbox{\tt DELANA}}
\newcommand{\DELSIM}{\mbox{\tt DELSIM}}
\newcommand{\DYMU}{\mbox{\tt DYMU3}}

% SPECIAL CHARACTERS %
\newcommand{\spot}{\mbox{$\bullet \;$}}


% CHI SQUAREDS %
\newcommand{\chindof}{\ensuremath{\chisq / \mathrm{dof}}}

% GROUPS %
% PARTICLES (and Z decays)%
\newcommand{\qqgam}{\ensuremath{q{\bar q}(\gamma)}}
\newcommand{\lplm}{\ensuremath{l^{+}l^{-}}}
\newcommand{\eell}{\ensuremath{\ee \ra \lplm}}
\newcommand{\nl}{\ensuremath{\nu_{l}}}
\newcommand{\nbl}{\ensuremath{{\overline{\nu}}_{l}}}
\newcommand{\Wp}{\ensuremath{\mathrm{W}^{+}}}
\newcommand{\Wm}{\ensuremath{\mathrm{W}^{-}}}
\newcommand{\W}{\ensuremath{\mathrm{W}}}
\newcommand{\Z}{\ensuremath{\mathrm{Z}}}
\newcommand{\ZZ}{\ensuremath{\mathrm{ZZ}}}
\newcommand{\Zee}{\ensuremath{\mathrm{Z \ee}}}
\newcommand{\Wen}{\ensuremath{\mathrm{W e \nel}}}
\newcommand{\Zgam}{\ensuremath{\mathrm{Z/\gamma}}}
\newcommand{\WW}{\ensuremath{\mathrm{ W^{+} W^{-} }}}

% W decay channels
\newcommand{\qqb}{\ensuremath{q{\bar q'}}}
\newcommand{\qbq}{\ensuremath{{\bar q}q'}}
\newcommand{\len}{\ensuremath{\l \nbl}}
\newcommand{\mn}{\ensuremath{\mu \nbmu}}
\newcommand{\en}{\ensuremath{e \nbel}}
\newcommand{\tn}{\ensuremath{\tau \nbtau}}
\newcommand{\nmn}{\ensuremath{{\overline{\mu}} \nmu}}
\newcommand{\nen}{\ensuremath{{\overline{e}} \nel}}
\newcommand{\ntn}{\ensuremath{{\overline{\tau}} \ntau}}

\newcommand{\qqqq}{\ensuremath{\mathrm{ \qqb \qbq}}} 
\newcommand{\lnqq}{\ensuremath{\mathrm{ \len  \qqb}}}
\newcommand{\enqq}{\ensuremath{\mathrm{ \en  \qqb}}}
\newcommand{\mnqq}{\ensuremath{\mathrm{ \mn  \qqb}}}
\newcommand{\tnqq}{\ensuremath{\mathrm{ \tn  \qqb}}}
\newcommand{\lnln}{\ensuremath{\l \nbl {\overline{\l}} \nl}}
\newcommand{\enen}{\ensuremath{\en \nen }}  
\newcommand{\mnmn}{\ensuremath{\mn \nmn}}
\newcommand{\tntn}{\ensuremath{\tn \ntn}}
\newcommand{\enmn}{\ensuremath{\en \nmn}}
\newcommand{\entn}{\ensuremath{\en \ntn}}
\newcommand{\mntn}{\ensuremath{\mn \ntn}}

% STANDARD MODEL PARAMS %
% W masses - pole mass, event masses
\newcommand{\mw}{\ensuremath{\mathrm{M_W}}}
\newcommand{\mwone}{\ensuremath{\mathrm{m_{\W 1}}}}
\newcommand{\mwtwo}{\ensuremath{\mathrm{m_{\W 2}}}}
\newcommand{\smw}{\ensuremath{\mathrm{m_W}}}
\newcommand{\mwav}{\ensuremath{\mathrm{\bar{m}_W}}}

\newcommand{\mz}{\ensuremath{\mathrm{M_Z}}}
\newcommand{\MZrp}[1]{\ensuremath{\mathrm{M_{\mbox{\tiny{Z}}}\!\!^{#1}}}}
\newcommand{\gz}{\ensuremath{\Gamma_{\mathrm{Z}}}}
\newcommand{\tz}{\ensuremath{\tau_{\mathrm{Z}}}}

\newcommand{\gw}{\ensuremath{\Gamma_{\mathrm{W}}}}
\newcommand{\mh}{\ensuremath{\mathrm{M_H}}}
\newcommand{\ssqtlef}{\ensuremath{{\sin}^{2}\theta^{\mathrm{eff}}_{l}}}
\newcommand{\gvl}{\ensuremath{g_{\mbox{\tiny V}}^{l}}}
\newcommand{\gal}{\ensuremath{g_{\mbox{\tiny A}}^{l}}}
\newcommand{\gvh}{\ensuremath{\hat{g}_{\mbox{\tiny V}}}}
\newcommand{\gah}{\ensuremath{\hat{g}_{\mbox{\tiny A}}}}
\newcommand{\mgen}{\ensuremath{\mathrm{M_{gen}}}}
%TGC%
\newcommand{\awphi}{\ensuremath{\alpha_{W\Phi}}}
\newcommand{\aw}{\ensuremath{\alpha_{W}}}
\newcommand{\abphi}{\ensuremath{\alpha_{B\Phi}}}
\newcommand{\dgz}{\ensuremath{\Delta g_{1}^{Z}}}
\newcommand{\dkap}{\ensuremath{\Delta\kappa_{\gamma}}}
\newcommand{\lamb}{\ensuremath{\lambda_{\gamma}}}
\newcommand{\twm}{\ensuremath{\theta_{W-}}}
\newcommand{\ctwm}{\ensuremath{\cos{\theta_{W-}}}}
\newcommand{\tfwm}{\ensuremath{\theta_{f}}}
\newcommand{\ctfwm}{\ensuremath{\cos{\theta_{f}}}}
\newcommand{\pfwm}{\ensuremath{\phi_{f}}}
\newcommand{\tfwp}{\ensuremath{\theta_{\bar{f}}}}
\newcommand{\ctfwp}{\ensuremath{\cos{\theta_{\bar{f}}}}}
\newcommand{\pfwp}{\ensuremath{\phi_{\bar{f}}}}
% ORDERS %
% OBSERVABLES %
\newcommand{\dsfbi}{\ensuremath{\delta\sigma_{\mbox{\tiny fb}}^{\mbox{\tiny int}}}}
\newcommand{\Afbmm}{\ensuremath{A_{\mbox{\tiny FB}}^{\mbox{\tiny $\mu\mu$}}}}
\newcommand{\Afbtt}{\ensuremath{A_{\mbox{\tiny FB}}^{\mbox{\tiny $\tau\tau$}}}}
\newcommand{\vcs}{\ensuremath{\left| V_{cs} \right|} }
\newcommand{\dsig}{\ensuremath{\frac{\mathrm{d}\sigma}{\mathrm{d}{\mathbf\Omega}}}}
\newcommand{\dsigob}{\ensuremath{\frac{\mathrm{d}\sigma}{\mathrm{d}\tilde{\mathbf\Omega}}}}

% KINEMATICS %
\newcommand{\prad}{\ensuremath{p_{\mbox{\tiny rad}}}}
\newcommand{\lambdabar}{\ensuremath{\lambda \! \! \! \! {\raisebox{+.5ex}{$-$}}}}

% PERIGEE PARAMETERS %
\newcommand{\rprg}{\ensuremath{r_{\mbox{\tiny p}}}}
\newcommand{\zprg}{\ensuremath{z_{\mbox{\tiny p}}}}
\newcommand{\thprg}{\ensuremath{\theta_{\mbox{\tiny p}}}}
\newcommand{\phprg}{\ensuremath{\phi_{\mbox{\tiny p}}}}

% UNITS %
\newcommand{\TeV}{\ensuremath{\mathrm{TeV}}}
\newcommand{\GeVm}{\ensuremath{\mathrm{GeV/c{^2}}}}
\newcommand{\GeVp}{\ensuremath{\mathrm{GeV/c}}}
\newcommand{\MeVm}{\ensuremath{\mathrm{MeV/c{^2}}}}
\newcommand{\KeV}{\ensuremath{\mathrm{KeV}}}
\newcommand{\eV}{\ensuremath{\mathrm{eV}}}
\newcommand{\um}{\ensuremath{\mathrm{m}}}
\newcommand{\uum}{\ensuremath{\mu{\mathrm m}}}
\newcommand{\ucm}{\ensuremath{\mathrm{cm}}}
\newcommand{\ufm}{\ensuremath{\mathrm{fm}}}
\newcommand{\umicrom}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\us}{\ensuremath{\mathrm{s}}}
\newcommand{\ums}{\ensuremath{\mathrm{ms}}}
\newcommand{\uus}{\ensuremath{\mu{\mathrm{s}}}}
\newcommand{\uns}{\ensuremath{\mathrm{ns}}}
\newcommand{\ups}{\ensuremath{\mathrm{ps}}}
\newcommand{\uub}{\ensuremath{\mu{\mathrm{b}}}}
\newcommand{\unb}{\ensuremath{\mathrm{nb}}}
\newcommand{\upb}{\ensuremath{\mathrm{pb}}}
\newcommand{\ipb}{\ensuremath{\mathrm{pb^{-1}}}}
\newcommand{\ifb}{\ensuremath{\mathrm{fb^{-1}}}}
\newcommand{\inb}{\ensuremath{\mathrm{nb^{-1}}}}

% SPECIAL TEXT %
\newcommand{\eg}{\mbox{\itshape e.g.}}
\newcommand{\etc}{\mbox{\itshape etc}}
\newcommand{\cf}{\mbox{\itshape cf.}}
\newcommand{\ffp}{\mbox{\itshape ff}}
\newcommand{\cm}{\mbox{c.m.}}
\newcommand{\ALEPH}{\mbox{\scshape Aleph}}
\newcommand{\DELPHI}{\mbox{\scshape Delphi}}
\newcommand{\OPAL}{\mbox{\scshape Opal}}
\newcommand{\LTHREE}{\mbox{\scshape L3}}
\newcommand{\CERN}{\mbox{\scshape Cern}}
\newcommand{\LEP}{\mbox{\scshape Lep}}
\newcommand{\LEPONE}{\mbox{\scshape Lep1}}
\newcommand{\LEPTWO}{\mbox{\scshape Lep2}}
\newcommand{\CDF}{\mbox{\scshape Cdf}}
\newcommand{\DO}{\mbox{\scshape D0}}
\newcommand{\SLD}{\mbox{\scshape Sld}}
\newcommand{\CLEO}{\mbox{\scshape Cleo}}
\newcommand{\UAONE}{\mbox{\scshape Ua1}}
\newcommand{\UATWO}{\mbox{\scshape Ua2}}
\newcommand{\TEVATRON}{\mbox{\scshape Tevatron}}
\newcommand{\LHC}{\mbox{\scshape LHC}}

\newcommand{\GENTLE}{\mbox{\ttfamily GENTLE}}
\newcommand{\TANAGRA}{\mbox{\ttfamily TANAGRA}}
\newcommand{\ZEBRA}{\mbox{\ttfamily ZEBRA}}
\newcommand{\PAW}{\mbox{\ttfamily PAW}}
\newcommand{\WWANA}{\mbox{\ttfamily WWANA}}
\newcommand{\FASTSIM}{\mbox{\ttfamily FASTSIM}}
\newcommand{\PYTHIA}{\mbox{\ttfamily PYTHIA}}
\newcommand{\JETSET}{\mbox{\ttfamily JETSET}}
\newcommand{\ARIADNE}{\mbox{\ttfamily ARIADNE}}
\newcommand{\HERWIG}{\mbox{\ttfamily HERWIG}}
\newcommand{\EXCALIBUR}{\mbox{\ttfamily EXCALIBUR}}
\newcommand{\ERATO}{\mbox{\ttfamily ERATO}}
\newcommand{\WPHACT}{\mbox{\ttfamily WPHACT}}
\newcommand{\CCTHREE}{\mbox{\ttfamily CC03}}
\newcommand{\NCEIGHT}{\mbox{\ttfamily NC08}}
\newcommand{\LUCLUS}{\mbox{\ttfamily LUCLUS}}
\newcommand{\JADE}{\mbox{\ttfamily JADE}}
\newcommand{\DURHAM}{\mbox{\ttfamily DURHAM}}
\newcommand{\CAMBRIDGE}{\mbox{\ttfamily CAMBRIDGE}}
\newcommand{\CONE}{\mbox{\ttfamily CONE}}
\newcommand{\PUFITC}{\mbox{\ttfamily PUFITC+}}
\newcommand{\PHDST}{\mbox{\ttfamily PHDST}}
\newcommand{\SKELANA}{\mbox{\ttfamily SKELANA}}
\newcommand{\DAFNE}{\mbox{\ttfamily DAFNE}}
\newcommand{\CERNLIB}{\mbox{\ttfamily CERNLIB}}
\newcommand{\MINUIT}{\mbox{\ttfamily MINUIT}}
\newcommand{\ELEPHANT}{\mbox{\ttfamily ELEPHANT}}
\newcommand{\GEANT}{\mbox{\ttfamily GEANT}}


% COMPOSITENESS %
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\erreps}{\ensuremath{\sigma_{\epsilon}}}
\newcommand{\errepsp}{\ensuremath{\sigma_{\epsilon}^{+}}}
\newcommand{\errepsm}{\ensuremath{\sigma_{\epsilon}^{-}}}
\newcommand{\Lmb}{\ensuremath{\Lambda}}
\newcommand{\lmb}{\ensuremath{\lambda}}
\newcommand{\Lmbsq}{\ensuremath{\Lambda^{2}}}
\newcommand{\Lmbisq}{\ensuremath{1/\Lambda^{2}}}
\newcommand{\Lmbpm}{\ensuremath{\Lambda^{\pm}}}
\newcommand{\Lmbp}{\ensuremath{\Lambda^{+}}}
\newcommand{\Lmbm}{\ensuremath{\Lambda^{-}}}
\newcommand{\gc}{\ensuremath{g_{c}}}
\newcommand{\etaij}{\ensuremath{\eta_{ij}}}


% lower case repeats - needed for bibtex
\newcommand{\gev}{\ensuremath{\mathrm{GeV}}}
\newcommand{\wpm}{\ensuremath{\mathrm{W}^\pm}}
\newcommand{\wm}{\ensuremath{\mathrm{W}^{-}}}
\newcommand{\w}{\ensuremath{\mathrm{W}}}
\newcommand{\z}{\ensuremath{\mathrm{Z}}}
\newcommand{\ww}{\ensuremath{\mathrm{ W^{+} W^{-} }}}
\newcommand{\tev}{\ensuremath{\mathrm{TeV}}}
\newcommand{\lep}{\mbox{\scshape Lep}}
\newcommand{\lepone}{\mbox{\scshape Lep1}}
\newcommand{\leptwo}{\mbox{\scshape Lep2}}
\newcommand{\delphi}{\mbox{\scshape Delphi}}
\newcommand{\excalibur}{\mbox{\ttfamily EXCALIBUR}}
\newcommand{\wwana}{\mbox{\ttfamily WWANA}}
\newcommand{\fastsim}{\mbox{\ttfamily FASTSIM}}
\newcommand{\phdst}{\mbox{\ttfamily PHDST}}
\newcommand{\skelana}{\mbox{\ttfamily SKELANA}}
\newcommand{\dafne}{\mbox{\ttfamily DAFNE}}
\newcommand{\delana}{\mbox{\ttfamily DELANA}}
\newcommand{\zebra}{\mbox{\ttfamily ZEBRA}}
\newcommand{\delsim}{\mbox{\ttfamily DELSIM}}
\newcommand{\pythia}{\mbox{\ttfamily PYTHIA}}
\newcommand{\jetset}{\mbox{\ttfamily JETSET}}
\newcommand{\ariadne}{\mbox{\ttfamily ARIADNE}}
\newcommand{\cdf}{\mbox{\scshape CDF}}
\newcommand{\gentle}{\mbox{\ttfamily GENTLE}}

%new commands for positioning especially in DELTEX
\newcommand{\bfl}{\begin{flushleft}}
\newcommand{\efl}{\end{flushleft}}
\newcommand{\bfr}{\begin{flushright}}
\newcommand{\efr}{\end{flushright}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

%bibliography stuff
\newcommand{\prd}[3]{Phys.\ Rev.\ {\bf D{#1}}, {#2} ({#3})}
\newcommand{\npb}[3]{Nucl.\ Phys.\ {\bf B{#1}}, {#2} ({#3})}
\newcommand{\plb}[3]{Phys.\ Lett.\ {\bf B{#1}}, {#2} ({#3})}
\newcommand{\zpc}[3]{Z. Phys.\ {\bf C{#1}}, {#2} ({#3})}
\newcommand{\prl}[3]{Phys.\ Rev.\ Lett.\ {\bf {#1}}, {#2} ({#3})}
\newcommand{\mpl}[3]{Mod.\ Phys.\ Lett.\ {\bf A{#1}}, {#2} ({#3})}
\newcommand{\ptp}[3]{Prog.\ Th.\ Phys.\  {\bf {#1}}, {#2} ({#3})}
\newcommand{\epj}[3]{Eur.\ Phys.\ J.  {\bf C{#1}}, {#2} ({#3})}
\newcommand{\jhep}[3]{JHEP {\bf {#1}}, {#2} ({#3})}
\newcommand{\hep}[1]{hep--ph/{#1}}
\newcommand{\yad}[3]{Yad.\ Fiz.\ {\bf{#1}}, {#2} ({#3})}
\newcommand{\pan}[3]{Phys.\ Atom.\ Nucl.\ {\bf{#1}}, {#2} ({#3})}
\newcommand{\sjn}[3]{Sov.\ J. Nucl.\ Phys.\ {\bf{#1}}, {#2} ({#3})}
\newcommand{\nca}[3]{Nuovo Cim.\ {\bf{#1}A}, {#2} ({#3})}
\newcommand{\jpg}[3]{J.\ Phys.\ G {\bf{#1}}, {#2} ({#3})}
\newcommand{\hip}[3]{Heavy Ion Phys.\ {\bf{#1}}, {#2} ({#3})}
\newcommand{\nim}[3]{Nucl.\ Instrum.\ Meth.\ {\bf A{#1}}, {#2} ({#3})}
\newcommand{\cpc}[3]{Comp.\ Phys.\ Comm.\  {\bf{#1}}, {#2} ({#3})}
\newcommand{\npps}[3]{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf{#1}}, {#2}
  ({#3})}
\newcommand{\lat}[1]{hep--lat/{#1}}
\newcommand{\ex}[1]{hep--ex/{#1}}
\newcommand{\ar}[3]{Annu.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf{#1}}, {#2}
    ({#3})}

%bphysics particles
\newcommand{\Bo}   {\ensuremath{\mathrm{B}^{0}_{\protect\mathrm{d}}}}
\newcommand{\Bobar}   {\ensuremath{\overline{\mathrm{B}^{0}_{\mathrm{d}}}}}
\newcommand{\Bod}   {\ensuremath{\mathrm{B}^{0}_{\protect\mathrm{d}}}}
\newcommand{\Bodbar}   {\ensuremath{\overline{\mathrm{B}^{0}_{\mathrm{d}}}}}
\newcommand{\Bos}   {\ensuremath{\mathrm{B}^{0}_{\protect\mathrm{s}}}}
\newcommand{\Bosbar}   {\ensuremath{\overline{\mathrm{B}^{0}_{\mathrm{s}}}}}
\newcommand{\rhoo}   {\ensuremath{\rho^{0}}}
\newcommand{\rhop}   {\ensuremath{\rho^{+}}}
\newcommand{\rhom}   {\ensuremath{\rho^{-}}}
\newcommand{\pio}   {\ensuremath{\pi^{0}}}
\newcommand{\pip}   {\ensuremath{\pi^{+}}}
\newcommand{\pim}   {\ensuremath{\pi^{-}}}
\newcommand{\pipm}   {\ensuremath{\pi^{\pm}}}

%Programs
\newcommand{\SICB} {\mbox{\ttfamily{SICB}}}

%Material 
\newcommand{\Xo}{\ensuremath{\mathrm{X}_{0}}}


==> layout_dbl.tex <==
%% ----------------------------------------------------------------------------
%% -- pjh_layout.tex ----------------------------------------------------------
%% ----------------------------------------------------------------------------
%%
%% ----------------------------------------------------------------------------
%% -- Oxford Thesis set-up ; single-sided, double-spaced ----------------------
%% ----------------------------------------------------------------------------
\setlength{\oddsidemargin}    {1.0cm}
\setlength{\evensidemargin}   {0.0cm}  % for double-sided printout
\setlength{\topmargin}        {-1.0cm}
\setlength{\headheight}       {1.0cm}
\setlength{\textwidth}        {15.0cm}
\setlength{\textheight}       {23.0cm}
%\baselineskip = 12pt plus 1pt minus 1pt   %single spaced
%\baselineskip = 24pt plus 1pt minus 1pt   %double spaced
\baselineskip = 21pt plus 1pt minus 1pt   % 1 3/4 spaced


==> layout_sgl.tex <==
%% ----------------------------------------------------------------------------
%% -- pjh_layout.tex ----------------------------------------------------------
%% ----------------------------------------------------------------------------
%%
%% ----------------------------------------------------------------------------
%% -- Oxford Thesis set-up ; single-sided, double-spaced ----------------------
%% ----------------------------------------------------------------------------
\setlength{\oddsidemargin}    {1.0cm}
\setlength{\evensidemargin}   {1.0cm}  % for single-sided printout
\setlength{\topmargin}        {-0.5cm}
\setlength{\headheight}       {1.0cm}
\setlength{\textwidth}        {15.0cm}
\setlength{\textheight}       {23.0cm}
%\baselineskip = 12pt plus 1pt minus 1pt   %single spaced
%\baselineskip = 24pt plus 1pt minus 1pt   %double spaced
\baselineskip = 21pt plus 1pt minus 1pt   % 1 3/4 spaced


==> preface.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                             %
%                               PREFACE                                       %
%                                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Preface}
%\thispagestyle{specialheadings}
%\rsectionmark{Preface}
\addcontentsline{toc}{chapter}{Preface}

Preface goes here. This gives a short overview/introduction
to the thesis as a whole, e.g. with a 1-paragraph intro, 
plus a paragraph per chapter.


==> refs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                          %%
%%                                 REFERENCES                               %%
%%                                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{References}
\baselineskip = 18pt plus 1pt minus 1pt   %this is 1 1/2 spaced
%\pagestyle{bibheadings}
%\thispagestyle{specialheadings}
\chaptermark{References}
\bibliography{referee}
\bibliographystyle{unsrt}


